Spatial quantum search in a triangular network

The spatial search problem consists in minimizing the number of steps required to find a given site in a network, under the restriction that only oracle queries or translations to neighboring sites are allowed. We propose a quantum algorithm for the spatial search problem on a triangular lattice with N sites and torus-like boundary conditions. The proposed algortithm is a special case of the general framework for abstract search proposed by Ambainis, Kempe and Rivosh [AKR05] (AKR) and Tulsi [Tulsi08], applied to a triangular network. The AKR-Tulsi formalism was employed to show that the time complexity of the quantum search on the triangular lattice is O(sqrt(N logN)).

==> mc2.tex <==
% more math commands
\newcommand{\ket}[1]{|#1\rangle}
\newcommand{\bra}[1]{\langle#1|}
\newcommand{\braket}[3]{\langle#1|#2|#3\rangle}
\newcommand{\scalar}[2]{\langle#1|#2\rangle}
\newcommand{\revbraket}[2]{|#1\rangle\langle#2|}
\newcommand{\op}[1]{|#1\rangle\langle#1|}
\newcommand{\opp}[2]{|#1\rangle\langle#2|}
%\newcommand{\spinor}[2]{{#1\choose #2}}
\newcommand{\spinor}[2]{\left(\begin{array}{c}#1\\#2\end{array}\right)}
\newcommand{\cn}{\frac{1}{\sqrt{2}}}
\newcommand{\order}[1]{{\mathcal O}\left(#1\right)}
\newcommand{\intk}{\int_{-\pi}^\pi \frac{dk}{2\pi}}
\newcommand{\intkk}{\intk\int_{-\pi}^\pi \frac{dk'}{2\pi}}
\newcommand{\imag}[1]{\mbox{Im}\left[#1\right]}
\newcommand{\real}[1]{\mbox{Re}\left[#1\right]}
\newcommand{\tr}[2]{\mbox{trace}_{#1}\left(#2\right)}


